StyleGAN-V: A Continuous Video Generator with the Price, Image Quality and Perks of StyleGAN2

Videos show continuous events, yet most $-$ if not all $-$ video synthesis frameworks treat them discretely in time. In this work, we think of videos of what they should be $-$ time-continuous signals, and extend the paradigm of neural representations to build a continuous-time video generator. For this, we first design continuous motion representations through the lens of positional embeddings. Then, we explore the question of training on very sparse videos and demonstrate that a good generator can be learned by using as few as 2 frames per clip. After that, we rethink the traditional image + video discriminators pair and design a holistic discriminator that aggregates temporal information by simply concatenating frames' features. This decreases the training cost and provides richer learning signal to the generator, making it possible to train directly on 1024$^2$ videos for the first time. We build our model on top of StyleGAN2 and it is just ${\approx}5\%$ more expensive to train at the same resolution while achieving almost the same image quality. Moreover, our latent space features similar properties, enabling spatial manipulations that our method can propagate in time. We can generate arbitrarily long videos at arbitrary high frame rate, while prior work struggles to generate even 64 frames at a fixed rate. Our model is tested on four modern 256$^2$ and one 1024$^2$-resolution video synthesis benchmarks. In terms of sheer metrics, it performs on average ${\approx}30\%$ better than the closest runner-up. Project website: https://universome.github.io.

==> algorithms/sampling.tex <==
\begin{algorithm}
\normalsize
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{A video $\bm x$, maximum distance between frames $D$, number of frames to sample $k$.}
\Output{A sequence of frames and their time locations.}

Compute the total number of frames in a video $L = \text{len}(\bm x)$\;
Randomly uniformly sample distance $d \sim U\{s\ |\ k \cdot 2^s \leq L \wedge 2^s \leq D\}$ \tcp*[l]{Logarithmically-distributed distances}
Randomly uniformly sample offset $\delta \sim U\{0, ..., D - kd\}$\;
Choose time locations $t_i = \delta + (i - 1) \cdot d$ for $i = 1, ..., k$\;
Extract $k$ frames from a video $\bm x_{t_i} = \bm x[t_i]$ for $i = 1, ..., k$\;
Return $(\bm x_{t_1}, ..., \bm x_{t_k}), (t_1, ..., t_k)$\;
\caption{Sample $k$ frames from a video to train \modelname{}.}
\label{alg:sampling}
\end{algorithm}

% \While{not converged}{
%     Sample a training batch $\bm X \subseteq D_\text{train}$\;
% %   \For{image $\bm x^{(i)} \in \bm X$}{
%     \For{$i\leftarrow 1$ \KwTo $|\bm X|$}{
%         Randomly sample side $s^{(i)} \in \{\text{left}, \text{right}\}$\;
%         % Cut the selected side $x^{(i)}_s$ (of size $H \times W/2 \times C$) from $x^{(i)}$\;
%         % Cut the selected half $\bm x^{(i)}_s$ from $x^{(i)}$\;
%         %   Split $x^{(i)}$ into two halves: $x^{(i)}_\text{left}$ and $x^{(i)}_\text{right}$\;
%         %   Randomly choose either $x^{(i)}_\text{left}$ or $x^{(i)}_\text{right}$\;
%         %   Assign label $y^{(i)} = 0$ for $x^{(i)}_\text{left}$ and $y^{(i)} = 1$ for $x^{(i)}_\text{right}$\;
%         %   Randomly select a training pair either $(x^{(i)}_\text{left}, 0)$ or $(x^{(i)}_\text{right}, 1)$\;
%         % Set label $y^{(i)} \leftarrow \mathds{1}[s = \text{right}]$\;
%         \eIf{$s^{(i)}$ = \textnormal{left}}{
%             $x^{(i)} \leftarrow x^{(i)}[:, :W/2]$ \tcp*[l]{Select the left half}
%             $y^{(i)} \leftarrow 0$\;
%         }{
%             $x^{(i)} \leftarrow x^{(i)}[:, W/2:]$ \tcp*[l]{Select the right half}
%             $y^{(i)} \leftarrow 1$\;
%         }
%   }
%   Update $C_\theta$ based on training batch $\{ x^{(i)}, y^{(i)} \}_{i=1}^{|\bm X|}$\;
% }


==> figures/fvd.tex <==
\begin{figure}
\centering
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fvd-scores.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fvd-scores.pdf}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/fvd-scores.pdf}
\end{subfigure}
\caption{Frechet Video Distance scores for different lengths on FaceForensics $256^2$, SkyTimelapse $256^2$ and Rainbow Jelly $256^2$. Our method performs much better for long videos, especially for complex datasets. We additionally highlight the FVD score}
\label{fig:fvd-scores}
\end{figure}


==> figures/motion-mapping-network.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{images/motion-mapping-network.pdf}
    \caption{Motion mapping network. We develop acyclic positional embeddings which depend on motion noise $\zm_{t_0}, ..., \zm_{t_n}, ...$ (see Sec~\ref{sec:method:generator} for details). It makes it possible to generate infinitely long aperiodic videos.}
    \label{fig:motion-mn}
\end{figure}

==> figures/motion-mode-collapse.tex <==
\begin{figure}
    \centering
    \includegraphics{Motion Mode Collapse. To the best of our knowledge, our work is the first one to explore \textit{motion mode collapse}, since the prior work didn't consider generating long videos.}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}

==> figures/old-architecture.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/generator.pdf}
    \caption{Generator architecture}
    \label{fig:architecture}
\end{figure*}


==> tables/main-ablations.tex <==
\begin{table*}[]
\caption{Ablating main components.}
\centering
% \resizebox{1.0\linewidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{FaceForensics} & \multicolumn{2}{c}{SkyTimelapse} & \multicolumn{2}{c}{UCF101} & \multicolumn{2}{c}{RainbowJelly} \\
& FVD$_{16}$ & FVD$_{128}$ & FVD$_{16}$ & FVD$_{128}$ & FVD$_{16}$ & FVD$_{128}$ & FVD$_{16}$ & FVD$_{128}$ \\
\midrule
\modelname\ \ours & 47.41 & 89.34 & 79.52 & 305.2 & 1431.0 & 1773.4 & 69.91 & 78.91 \\
~$-$ continuous-time $\G$ & 65.88 & 41.77 & 109.1 & 110.2 & 0.0 & 0.0 & 0.0 & 0.0 \\
~$-$ hypernet-based $\D$ & 154.0 & 139.1 & 236.9 & 258.0 & 0.0 & 0.0 & 0.0 & 0.0 \\
~$-$ long-range sampling & 55.62 & 309.3 & 85.88 & 272.8 & 0.0 & 0.0 & 0.0 & 0.0 \\
\bottomrule
\end{tabular}
% }
\end{table*}


==> tables/motion-codes.tex <==
\begin{table}
\caption{Ablating motion codes .}
\label{table:compute}
\centering
% \resizebox{1.0\linewidth}{!}{
\begin{tabular}{lccc}
\toprule
Method & train time & \#img/sec & mem \\ 
\midrule
MoCoGAN \cite{MoCoGAN} & 0.0 & 0.0 \\
~+ StyleGAN2 backbone & 0.0 & 0.0 \\
MoCoGAN-HD \cite{MoCoGAN-HD} & 0.0 & 0.0 \\
VideoGPT \cite{VideoGPT} & 0.0 & 0.0 \\
DIGAN \cite{DIGAN} & 0.0 & 0.0 \\
\midrule
\modelname\ \ours & 0.0 & 0.0 \\
\bottomrule
\end{tabular}
% }
\end{table}

